Almost Tight Approximation Hardness for Single-Source Directed k-Edge-Connectivity

In the $k$-connected directed Steiner tree problem ($k$-DST), we are given an $n$-vertex directed graph $G=(V,E)$ with edge costs, a connectivity requirement $k$, a root $r\in V$ and a set of terminals $T\subseteq V$. The goal is to find a minimum-cost subgraph $H\subseteq G$ that has $k$ internally disjoint paths from the root vertex $r$ to every terminal $t\in T$. In this paper, we show the approximation hardness of $k$-DST for various parameters, which thus close some long-standing open problems. - $\Omega\left(|T|/\log |T|\right)$-approximation hardness, which holds under the standard assumption $\mathrm{NP}\neq \mathrm{ZPP}$. The inapproximability ratio is tightened to $\Omega\left(|T|\right)$ under the Strongish Planted Clique Hypothesis [Manurangsi, Rubinstein and Schramm, ITCS 2021]. The latter hardness result matches the approximation ratio of $|T|$ obtained by a trivial approximation algorithm, thus closing the long-standing open problem. - $\Omega\left(\sqrt{2}^k / k\right)$-approximation hardness for the general case of $k$-DST under the assumption $\mathrm{NP}\neq\mathrm{ZPP}$. This is the first hardness result known for survivable network design problems with an inapproximability ratio exponential in $k$. - $\Omega\left((k/L)^{L/4}\right)$-approximation hardness for $k$-DST on $L$-layered graphs for $L\le O\left(\log n\right)$. This almost matches the approximation ratio of $O(k^{L-1}\cdot L \cdot \log |T|)$ achieving in $O\left(n^L\right)$-time due to Laekhanukit [ICALP`16].

==> warm-up.tex <==
\section{Warming up}

% We use a simple example to explain our reduction.
% Let $(\+G,\Sigma,\pi)$ be a Label Cover instance where $\+G=(\+U,\+W,\+E)$ is the graph in \Cref{fig:TerminalLabelCover}, $\Sigma=\set{1,2}$ and $\pi_{u_i,w_j}:\Sigma \to \Sigma$ is the identity function for each edge $(u_i, w_j)\in \+E$.
% Although this is a trivial example from label cover's point of view, it is enough to demonstrate the nontrivial ideas used in our reduction.
% We construct a directed graph $G$ of the $k$-DST problem from $(\+G,\Sigma,\pi)$ as follows.

% \tikzset{
%   vertex/.style= {
%     circle,
%     draw,
%     line width = .5mm,
%     color = black,
%     minimum size = 1.1cm
%     }
% }

% \usetikzlibrary{graphs}

% \begin{figure}[htbp]
%   \centering
%   \begin{tikzpicture}
%     \node[vertex] (w1) at (0,0){$w_1$};
%     \node[vertex] (w2) at (3,0){$w_2$};
%     \node[vertex] (u1) at (0,2){$u_1$};
%     \node[vertex] (u2) at (3,2){$u_2$};
%     \draw[line width = \LW] (u1) -- (w1) -- (u2) -- (w2);
%   \end{tikzpicture}
%   \caption{Label cover : a bipartite graph $G=(\+U\cup\+W, \+E)$ where $\+U=\set{u_1,u_2}$ and $\+W=\set{w_1,w_2}$.}
%   \label{fig:TerminalLabelCover}
% \end{figure}

% %Let $\sigma$ a multi-labeling of $\+G$.
% %Rewrite the edge set $\+E$ as disjoint unions of matchings, that is, $\+E=\set{u_1w_1, u_2w_2}\cup \set{u_2 w_1}\equiv \+E_1\cup \+E_2$.
% %In the general case, we can use \Cref{lem:matching} to decompose $\+E$ into at most $\Delta$ matchings, where $\Delta$ is the maximum degree of the label cover instance.
% \begin{enumerate}
%   \item Let $G$ be a graph with a single vertex $r$ as the root.
%         For $i\in \set{1,2}$ and $a\in \Sigma=\set{1,2}$, add a vertex $u_{i,a}$ to $G$ and add an edge from $r$ to $u_{i,a}$ of cost $1$.
%         See \Cref{fig:TerminalDST-1} for an illustration.
%         Intuitively, we use the edge $r\to u_{i,a}$ to encode whether $a$ is contained in the multilabeling at $u_i$, that is, if the edge $r\to u_{i,a}$ is (not) contained in a solution then $a$ is (not) contained in the corresponding multilabeling at $u_i$.

%   \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%     \end{tikzpicture}
%     \caption{Construct the root.}
%     \label{fig:TerminalDST-1}
%   \end{figure}

%   \item Then we apply similar gadgets to $w_j\in \+W$.
%         For each $j\in \set{1,2}$, add a vertex $w_j$ to $G$.
%         For each $j\in \set{1,2}$ and $a\in \Sigma$, add a vertex $w_{j,a}$ to $G$ and add an edge from $w_{j,a}$ to $w_j$ of cost $1$.
%         See \Cref{fig:TerminalDST-2} for an illustration.
%         We remark that all the edges in the reduction with positive costs have been given, that is, all the edges added hereafter are of cost zero.

%   \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-4.5){$w_1$};
%       \node[vertex] (w2) at (2.25,-4.5){$w_2$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%     \end{tikzpicture}
%     \caption{}
%     \label{fig:TerminalDST-2}
%   \end{figure}

%   \item We also need to implement the edges $\set{u_1w_1, u_2w_1, u_2w_2}$ and the constraints on them in certain way.
%   For each edge $u_iw_j$ and $a,b\in \Sigma$, add an edge from $u_{i,a}$ and $w_{j,b}$ if $\pi_{u_iw_j}(a)=b$.
%   See \Cref{fig:TerminalDST-3} for an illustration.
%   This construction is part of the gadget that encodes whether a constraint $\pi_{u_iw_j}$ is satisfied.
%   More concretely, we want the path $r\to u_{i,a} \to w_{j,b} \to w_j$ to correspond to $\pi_{u_iw_j}(a)=b$.

%   \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \draw[->, line width = \LW] (u12) -- (w12);
%       \draw[->, line width = \LW] (u21) -- (w21);
%       \draw[->, line width = \LW] (u22) -- (w22);
%       \draw[->, line width = \LW] (u21) -- (w11);
%       \draw[->, line width = \LW] (u22) -- (w12);
%     \end{tikzpicture}
%     \caption{}
%     \label{fig:TerminalDST-3}
%   \end{figure}

%   \item To really make the gadget work, we need to add terminals and set the connectivity requirement $k$.
%   Write the edges as $\+E=\set{u_1w_1, u_2w_2}\cup \set{u_2 w_1}\equiv \+E_1\cup \+E_2$.
%   Note that both $\+E_1$ and $\+E_2$ are matchings.
%   Add two terminals $t_1$ and $t_2$.
%   For each $l\in\set{1,2}$ and $u_i w_j\in \+E_l$, add an edge from $w_j$ to terminal $t_l$.
%   See \Cref{fig:TerminalDST-4} for an illustration.
%   In general, we can use \Cref{lem:matching} to decompose $\+E$ into at most $\Delta$ matchings, where $\Delta$ is the maximum degree of the underlying graph in the label cover instance.
%   Then we set a terminal $t_l$ for each matching and thus the number of terminals is at most $\Delta$.

%   \begin{figure}[htbp]
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \draw[->, line width = \LW] (u12) -- (w12);
%       \draw[->, line width = \LW] (u21) -- (w21);
%       \draw[->, line width = \LW] (u22) -- (w22);
%       \draw[->, line width = \LW] (u21) -- (w11);
%       \draw[->, line width = \LW] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w2) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%     \end{tikzpicture}
%     \caption{}
%     \label{fig:TerminalDST-4}
%     \end{minipage}
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u11) -- (w11);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u12) -- (w12);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u21) -- (w21);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u22) -- (w22);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u21) -- (w11);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w1) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w2) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w1) -- (t2);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) to [bend right=25] (t2);
%     \end{tikzpicture}
%     \caption{}
%     \label{fig:TerminalDST-buy-edges}
%     \end{minipage}
%   \end{figure}

%   If we set $k=2$ for this example and add a dummy edge of cost zero from $r$ to $t_2$, then the completeness is already satisfied.
%   This means that for any feasible multilabeling $\sigma$ of the label cover instance, there is a corresponding feasible subgraph of $G$ with the same cost.
%   For example, let $\sigma$ be the multilabeling where each vertex $u\in \+U\cup \+W$ is assigned $\set{1}$.
%   Let $H$ be a subgraph where $V(H)=V(G)$.
%   Add the zero cost edges in $G$ (black edges in \Cref{fig:TerminalDST-4}), including the dummy edge from $r$ to $t_2$, to $H$.
%   Then add the edges $\set{r\to u_{i,1}}_{i=1,2}$ and $\set{w_{j,1}\to w_j}_{j=1,2}$ to $H$.
%   See \Cref{fig:TerminalDST-buy-edges} for an illustration where the edges of $H$ are bold orange.
%   Clearly the cost of $H$ is exactly $4 = \cost(\sigma)$.
%   It is easy to verify that there are two edge disjoint paths from $r$ to $t_1$ (see \Cref{fig:TerminalDST-t1}) and to $t_2$ (see \Cref{fig:TerminalDST-t2}).

%   \begin{figure}[htbp]
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = 2*\LW, color=YellowGreen] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (u11) -- (w11);
%       \draw[->, line width = \LW] (u12) -- (w12);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (u21) -- (w21);
%       \draw[->, line width = \LW] (u22) -- (w22);
%       \draw[->, line width = \LW] (u21) -- (w11);
%       \draw[->, line width = \LW] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w1) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w2) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%       \draw[->, line width = \LW] (r) to [bend right=25] (t2);
%     \end{tikzpicture}
%     \caption{Two edge-disjoint paths from $r$ to $t_1$}
%     \label{fig:TerminalDST-t1}
%     \end{minipage}
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \draw[->, line width = \LW] (u12) -- (w12);
%       \draw[->, line width = \LW] (u21) -- (w21);
%       \draw[->, line width = \LW] (u22) -- (w22);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (u21) -- (w11);
%       \draw[->, line width = \LW] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w2) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (w1) -- (t2);
%       %\draw (r) arc[start angle=40, delta angle=0] -- (t2);
%       \draw[->, line width = 2*\LW, color=YellowGreen] (r) to [bend right=25] (t2);
%     \end{tikzpicture}
%     \caption{Two edge-disjoint paths from $r$ to $t_2$}
%     \label{fig:TerminalDST-t2}
%     \end{minipage}
%   \end{figure}

%   \begin{figure}[htbp]
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5,-1.5){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5,-1.5){$u_{2,1}$};
%       \node[vertex] (u22) at (3,-1.5){$u_{2,2}$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) -- (u22);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5,-3.5){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5,-3.5){$w_{2,1}$};
%       \node[vertex] (w22) at (3,-3.5){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \node[vertex] (w2) at (2.25,-5){$w_2$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w22) -- (w2);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u11) -- (w11);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u12) -- (w12);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u21) -- (w21);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u22) -- (w22);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u21) -- (w11);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w1) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w2) -- (t1);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (w1) -- (t2);
%       \draw[->, line width = 2*\LW, color=YellowOrange] (r) to [bend right=25] (t2);
%     \end{tikzpicture}
%     \centering
%     \caption{}
%     \label{fig:infeasible}
%   \end{figure}

%   However, if we stop here the soundness is not true.
%   Let $H$ be a feasible subgraph of $G$.
%   There is a natural way to map $H$ back to a multilabeling $\sigma$ of $\+G$ as follows: let $\sigma(u_i) = \set{a: r\to u_{i,a}\in E(H)}$ and $\sigma(w_j) = \set{b: w_{j,b}\to w_j \in E(H)}$.
%   If $H$ consists of the bold orange edges in \Cref{fig:infeasible}, then it is feasible but the corresponding multilabeling $\sigma$ is infeasible.
%   The reason is that when we add the terminal $t_2$, we want a path of the form $r\to u_{2,\star} \to w_{1,\star} \to w_1 \to t_2$ which mimics the constraint $\pi_{u_2w_1}$.
%   Unfortunately, it is possible to use a path of the form $r\to u_{1,\star} \to w_{1,\star} \to w_1 \to t_2$ to get a path from $r$ to $t_2$.
%   We will use a small gadget to fix the problem for terminal $t_2$ while (essentially) not adding new paths from the root to other terminals.

%   \item
%   Suppose we want to make the path $r\to u_{1,1} \to w_{1,1} \to w_1 \to t_2$ invalid (see \Cref{fig:small-gadget-1}).
%   We can add new edges $r\to u_{1,1}$ and $w_{1,1} \to t_2$ of cost zero and set $k=3$ (see \Cref{fig:small-gadget-2}).
%   Since $t_2$ has exactly $3$ incoming edges and $k=3$, a feasible subgraph $H$ must contain the edge $w_{1,1} \to t_2$.
%   By tracing back, the path $r\to u_{1,1} \to w_{1,1} \to t_2$ of cost zero (or cost one if we choose the blue edge $r\to u_{1,1}$) must be contained in $H$.
%   Since the edge $u_{1,1} \to w_{1,1}$ is used, the edge-disjointness requirement for paths from $r$ to $t_2$ make the path $r\to u_{1,1}\to w_{1,1} \to w_1 \to t_2$ of cost $2$ infeasible.
%   However, since we add an edge from $r$ to $u_{1,1}$, there are new unwanted paths from $r$ to $t_1$.
%   Note that the edge $w_{1,1}\to t_2$ dose not create new paths from $r$ to terminals other than $t_2$, because it is an edge with a terminal as an ending point.
%   We can fix this via a simple trick.
%   We add a zero cost edge from $u_{1,1}$ to $t_1$ (see \Cref{fig:small-gadget-3}).

%   \begin{figure}[htbp]
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       %\node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       %\draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%     \end{tikzpicture}
%     \caption{A path to forbid}
%     \label{fig:small-gadget-1}
%     \end{minipage}
%     \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%       \draw[->, line width = 2*\LW] (r) to [bend right=25] (u11);
%       \draw[->, line width = 2*\LW] (w11) to [bend left=25] (t2);
%     \end{tikzpicture}
%     \caption{Make $u_{1,1}\to w_{1,1}$ invalid for $t_2$}
%     \label{fig:small-gadget-2}
%     \end{minipage}
%   \end{figure}

%   \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3,-1.5){$u_{1,1}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \node[vertex] (w11) at (-3,-3.5){$w_{1,1}$};
%       \node[vertex] (w1) at (-2.25,-5){$w_1$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \node[vertex] (t1) at (-2.25, -7) {$t_1$};
%       \node[vertex] (t2) at ( 2.25, -7) {$t_2$};
%       \draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%       \draw[->, line width = 2*\LW] (r) to [bend right=25] (u11);
%       \draw[->, line width = 2*\LW] (w11) to [bend left=25] (t2);
%       \draw[->, line width = 2*\LW] (u11) to [bend right=40] (t1);
%     \end{tikzpicture}
%     \caption{The final gadget}
%     \label{fig:small-gadget-3}
%   \end{figure}

%   \item Applying the gadget to each terminals, we obtained the $k$-DST instance ($k=6$, see \Cref{fig:final-instance}).
%   The black, green and orange edges are of cost zero and the blue edges are of cost one.
%   There is a natural one-to-one mapping without changing the cost between the feasible multilabeling $\sigma$ of $\+G$ and feasible subgraphs $H$ of $(k,G,r,T)$ (assuming that all zero-cost edges are contained in $H$).

%   \begin{figure}[htbp]
%     \centering
%     \begin{tikzpicture}
%       \node[vertex] (r) at (0,0){$r$};
%       \node[vertex] (u11) at (-3*\scale,-1.5*\scale){$u_{1,1}$};
%       \node[vertex] (u12) at (-1.5*\scale,-1.5*\scale){$u_{1,2}$};
%       \node[vertex] (u21) at (1.5*\scale,-1.5*\scale){$u_{2,1}$};
%       \node[vertex] (u22) at (3*\scale,-1.5*\scale){$u_{2,2}$};
%       \draw[->, line width = \LW, color=blue] (r) -- (u11);
%       \draw[->, line width = \LW, color=blue] (r) -- (u12);
%       \draw[->, line width = \LW, color=blue] (r) -- (u21);
%       \draw[->, line width = \LW, color=blue] (r) -- (u22);
%       \node[vertex] (w11) at (-3*\scale,-3.5*\scale){$w_{1,1}$};
%       \node[vertex] (w12) at (-1.5*\scale,-3.5*\scale){$w_{1,2}$};
%       \node[vertex] (w21) at (1.5*\scale,-3.5*\scale){$w_{2,1}$};
%       \node[vertex] (w22) at (3*\scale,-3.5*\scale){$w_{2,2}$};
%       \node[vertex] (w1) at (-2.25*\scale,-5*\scale){$w_1$};
%       \node[vertex] (w2) at (2.25*\scale,-5*\scale){$w_2$};
%       \draw[->, line width = \LW, color=blue] (w11) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w12) -- (w1);
%       \draw[->, line width = \LW, color=blue] (w21) -- (w2);
%       \draw[->, line width = \LW, color=blue] (w22) -- (w2);
%       \draw[->, line width = \LW] (u11) -- (w11);
%       \draw[->, line width = \LW] (u12) -- (w12);
%       \draw[->, line width = \LW] (u21) -- (w21);
%       \draw[->, line width = \LW] (u22) -- (w22);
%       \draw[->, line width = \LW] (u21) -- (w11);
%       \draw[->, line width = \LW] (u22) -- (w12);
%       \node[vertex] (t1) at (-2.25*\scale, -7*\scale) {$t_1$};
%       \node[vertex] (t2) at ( 2.25*\scale, -7*\scale) {$t_2$};
%       \draw[->, line width = \LW] (w1) -- (t1);
%       \draw[->, line width = \LW] (w2) -- (t1);
%       \draw[->, line width = \LW] (w1) -- (t2);
%       \draw[->, line width = \LW] (r) to [bend right=15] (t2);

%       \draw[->, line width = \LW, color=YellowGreen] (r) to [bend right=25] (u11);
%       \draw[->, line width = \LW, color=YellowGreen] (u11) to [bend right=40] (t1);
%       \draw[->, line width = \LW, color=YellowGreen] (w11) to (t2);

%       \draw[->, line width = \LW, color=YellowGreen] (r) to [bend left=25] (u12);
%       \draw[->, line width = \LW, color=YellowGreen] (u12) to [bend left=40] (t1);
%       \draw[->, line width = \LW, color=YellowGreen] (w12) to (t2);

%       \draw[->, line width = \LW, color=YellowOrange] (r) to [bend right=25] (u21);
%       \draw[->, line width = \LW, color=YellowOrange] (w11) to [bend right=15] (t1);
%       \draw[->, line width = \LW, color=YellowOrange] (u21) to [bend right=40] (t2);

%       \draw[->, line width = \LW, color=YellowOrange] (r) to [bend left=25] (u22);
%       \draw[->, line width = \LW, color=YellowOrange] (w12) to [bend left=15] (t1);
%       \draw[->, line width = \LW, color=YellowOrange] (u22) to [bend left=40] (t2);
%     \end{tikzpicture}
%     \caption{Final instance}
%     \label{fig:final-instance}
%   \end{figure}
% \end{enumerate}

